Task Preference Optimization: Improving Multimodal Large Language Models with Vision Task Alignment

Current multimodal large language models (MLLMs) struggle with fine-grained or precise understanding of visuals although they give comprehensive perception and reasoning in a spectrum of vision applications. Recent studies either develop tool-using or unify specific visual tasks into the autoregressive framework, often at the expense of overall multimodal performance. To address this issue and enhance MLLMs with visual tasks in a scalable fashion, we propose Task Preference Optimization (TPO), a novel method that utilizes differentiable task preferences derived from typical fine-grained visual tasks. TPO introduces learnable task tokens that establish connections between multiple task-specific heads and the MLLM. By leveraging rich visual labels during training, TPO significantly enhances the MLLM's multimodal capabilities and task-specific performance. Through multi-task co-training within TPO, we observe synergistic benefits that elevate individual task performance beyond what is achievable through single-task training methodologies. Our instantiation of this approach with VideoChat and LLaVA demonstrates an overall 14.6% improvement in multimodal performance compared to baseline models. Additionally, MLLM-TPO demonstrates robust zero-shot capabilities across various tasks, performing comparably to state-of-the-art supervised models. The code will be released at https://github.com/OpenGVLab/TPO

==> tables/ablate_mvbench.tex <==
\begin{table}[ht]
\caption{Ablation of TPO method on LLaVA-OneVison-7B\cite{li2024llava}.}
  \centering
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{l|cc}
    \toprule
    Model &   LLaVA-OneVison &  LLaVA-OneVison-TPO  \\
    \midrule
    MVBench & 56.7  &  64.8      \\ 
    \bottomrule
    \end{tabular}
}
\label{tab:ablate_mvbench}
\end{table}

==> tables/full_videomme.tex <==

\begin{table}[h]
\caption{Performance comparison of MLLMs on Video-MME. w/o s. means without subtitle and w s. means with subtitle. F indicates the number of frames.}
  \centering
  \resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|cc|cc|cc|cc}
    \toprule
    
    \multirow{2}{*}{Model} &  \multirow{2}{*}{F} & \multicolumn{2}{c}{Overall}
    & \multicolumn{2}{c}{Short } & \multicolumn{2}{c}{Medium } & \multicolumn{2}{c}{Long }\\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6}  \cmidrule(lr){7-8} \cmidrule(lr){9-10} 
    &  & w/o s.  & w s. & w/o s.  & w s. & w/o s.  & w s. & w/o s.  & w s. \\  
    \midrule 
    VideoChat2~\cite{mvbench}  & 16  & 39.5 & 43.8 & 48.3 & 52.8 & 37.0 &39.4 &33.2 &39.2\\ 
    Video-LLaVA~\cite{video-llava} & 8 & 39.9 & 41.6 &45.3&46.1& 38.0& 40.7 & 36.2 & 38.1\\  
    ST-LLM~\cite{st-llm}   & 64   & 39.9 & 43.6  & 45.7 & 48.7 & 36.8 & 41.4 & 31.3 & 36.9\\ 
    Chat-UniVi~\cite{jin2023chatunivi} & 64 & 40.6&	45.9  & 45.7 & 51.2 & 40.3 & 44.6 & 35.8 & 41.8\\
    ShareGemini~\cite{ShareGemini} &64 & 43.2 &47.9 & 49.1 & 52.8 & 41.3 & 47.3 & \textbf{39.1} & 43.4\\
    \midrule 
    VideoChat-TPO & 16  &\textbf{46.2} & \textbf{51.5}  & \textbf{54.9} & \textbf{60.8} & \textbf{42.6} & \textbf{48.0} & \textbf{41.1} & \textbf{45.8}\\ 
    \bottomrule
    \end{tabular}
}
\label{atab:videomme}
\end{table}


==> tables/image_benchmark.tex <==
\begin{table*}[ht]
% \caption{Results on NExT-GQA. Acc@IoP indicates the percentage of correct answers when the IoP $\geq$ 0.5. Acc@GQA is defined as the percentage of questions that are both correctly answered and visually grounded with IoP $\geq$ 0.5.}
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|c|c}
    \toprule
    Model & MMIU~\cite{meng2024mmiu} & SEED2$_{I}$~\cite{seedbench2} & SEED2$_{M}$~\cite{seedbench2} \\
    \midrule 
    LLaVA-v1.5-7b~\cite{llava}  & 19.2  & 58.3  & 39.2  \\  
    ShareGPT4V-7b~\cite{sharegpt4v} & 18.5 & - & - \\
    OpenFlamingo~\cite{awadalla2023openflamingo} & 22.3 & 36.6  & 43.5 \\
    LLaVA-Interleave~\cite{li2024llava}  & 32.4 & -  & - \\
    VideoChat2~\cite{mvbench}    & 35.0 & 26.5  & 27.6 \\ 
    VideoChatGPT~\cite{video-chatgpt} & - & 38.3 & 49.8 \\
    InternLM-XComposer~\cite{ixc2} & 21.9 & 65.4  & 49.8 \\
    \midrule  
    VideoChat-TPO  &\textbf{40.2}~\textcolor{olive}{(+5.2)}   & \textbf{67.3}~\textcolor{olive}{(+40.9)}  &  \textbf{70.0}~\textcolor{olive}{(+42.4)}  \\ 
    \bottomrule
    \end{tabular}
    }
\caption{\textbf{Performance on Image Understanding.} }%Compared to the 7B parameter model, the TPO-optimized model enhanced image understanding performance, especially in multi-image scenarios.}
\label{tab:MMIU}
\end{table*}


        

==> tables/mmiu_mlvu.tex <==
\begin{table}[th]
\caption{\textbf{Performance on Multimodal Multi-image Understanding.} Compared to the 7B parameter model, the TPO-optimized model enhanced image understanding performance, especially in multi-image scenarios.}
  \centering
  \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|c|c|c}
    \toprule
    
    Model & MMIU~\cite{meng2024mmiu} & SEED2$_{image}$~\cite{seedbench2} & SEED2$_{multi}$~\cite{seedbench2} \\
    \midrule 
    LLaVA-v1.5-7b~\cite{llava}  & 19.2  & 58.3  & 39.2  \\  
    ShareGPT4V-7b~\cite{sharegpt4v} & 18.5 & - & - \\
    
    OpenFlamingo~\cite{awadalla2023openflamingo} & 22.3 & 36.6  & 43.5 \\
    LLaVA-Interleave~\cite{li2024llava}  & 32.4 & -  & - \\
    VideoChat2~\cite{mvbench}    & 35.0 & 26.1  & 27.6 \\ 
    VideoChatGPT~\cite{video-chatgpt} & - & 38.3 & 49.8 \\
    InternLM-XComposer~\cite{ixc2} & 21.9 & 65.4  & 49.8 \\
    \midrule  
    VideoChat-TPO  &\textbf{40.2}   & \textbf{67.3}  &  \textbf{70.0}  \\ 
    \bottomrule
    \end{tabular}
}
\label{tab:MMIU}
\end{table}



==> tables/moment_retrieval_ft.tex <==
\begin{table}[ht]
\caption{\textbf{Fine-tuning Performance on moment retrieval and highlight detection tasks.}}
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc|c|cc}
    \toprule
    \multirow{2}{*}{Model} &\multicolumn{4}{c}{Charades-STA~\cite{charades-sta}} &\multicolumn{2}{|c}{QVHighlight~\cite{qvhighlight}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-7}
    &R@0.3 &R@0.5 &R@0.7 &mIoU &mAP &HIT@1\\
    \midrule 
    M-DETR~\cite{m-detr}    & 65.8 & 52.1  & 30.6 & 45.5 & 35.7  & 55.6  \\
    QD-DETR~\cite{qd-detr}  & -    & 57.3  & 32.6 & -    & 38.9  & 62.4 \\
    UniVTG~\cite{univtg}    & 72.6 & 60.2  & 38.6 & 52.2 & \textbf{40.5}  & \textbf{66.3} \\
    \midrule
    TimeChat~\cite{Ren2023TimeChat}& - & 46.7 & 23.7 & -    & 21.7 & 37.9  \\
    HawkEye~\cite{hawkeye}      & 72.5 & 58.3 & 28.8 & - & - & -\\
    \midrule 
     \ModelName   & \textbf{77.0} & \textbf{65.0} & \textbf{40.7} & \textbf{55.0} & 38.6 & 65.4\\  
    \bottomrule 
\end{tabular}
}
\label{tab:tvg_ft}
\end{table}

==> tables/moment_retrieval_zs.tex <==
\begin{table}[h]
\caption{\textbf{Zero-shot Performance on moment retrieval task.}}
  \centering
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{l|ccc|c}
    \toprule
    
    \multirow{2}{*}{Model} &\multicolumn{4}{c}{Charades-STA~\cite{}} \\
    \cmidrule(lr){2-5} &R@0.3 &R@0.5 &R@0.7 &mIoU\\
    \midrule 
    UniVTG~\cite{univtg} & 44.1 & 25.2  & 10.0 & 27.1 \\
    \midrule 
    Video-ChatGPT~\cite{video-chatgpt} & 27.2 & 6.2  & 1.9 & 19.7\\
    Valley~\cite{valley}    & 28.4 & 1.8  & 0.3 & 21.4\\
    VideoChat~\cite{videochat} & 32.8 & 8.6  & 0.0  & 25.9\\
    VideoChat2~\cite{mvbench}& 38.0 & 14.3 & 3.8  & 24.6\\
    \midrule
    VTimeLLM~\cite{vtimellm}  & 51.0 & 27.5 & 11.4 & 31.2\\
    TimeChat~\cite{Ren2023TimeChat}  & -    & 32.2 & 13.4 & -   \\
    HawkEye~\cite{hawkeye}   & 50.6 & 31.4 & 14.5 & 33.7 \\
    ChatVTG ~\cite{chatvtg}         &52.7 & 33.0 & 15.9 &34.9 \\      
    \midrule 
    \ModelName   & \textbf{58.3} & \textbf{40.2} & \textbf{18.4} & \textbf{38.1}\\  
    \bottomrule 
\end{tabular}
}
\label{tab:tvg_zs}
\end{table}

==> tables/mvbench.tex <==
\begin{table*}[ht]
\caption{Results on MVBench multi-choice question answering.}
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|cccccccccccccccccccc}
    \toprule
    Model &Avg. &AS &AP &AA &FA &UA &OE &OI &OS &MD &AL &ST &AC &MC &MA &SC &FP &CO &EN &ER &CI \\
    \midrule 
    % Otter-V \citep{otter}              & \cellcolor{gray!10}{26.8} & 23.0 & 23.0 & 27.5 & 27.0 & 29.5 & 53.0 & 28.0 & 33.0 & 24.5 & 23.5 & 27.5 & 26.0 & 28.5 & 18.0 & 38.5 & 22.0 & 22.0 & 23.5 & 19.0 & 19.5 \\
    % mPLUG-Owl-V \citep{mplug-owl}      & \cellcolor{gray!10}{29.7} & 22.0 & 28.0 & 34.0 & 29.0 & 29.0 & 40.5 & 27.0 & 31.5 & 27.0 & 23.0 & 29.0 & 31.5 & 27.0 & 40.0 & 44.0 & 24.0 & 31.0 & 26.0 & 20.5 & 29.5 \\
    VideoChatGPT \citep{video-chatgpt} & 32.7 & 23.5 & 26.0 & 62.0 & 22.5 & 26.5 & 54.0 & 28.0 & 40.0 & 23.0 & 20.0 & 31.0 & 30.5 & 25.5 & 39.5 & 48.5 & 29.0 & 33.0 & 29.5 & 26.0 & 35.5 \\
    VideoLLaMA \citep{video-llama}     & 34.1 & 27.5 & 25.5 & 51.0 & 29.0 & 39.0 & 48.0 & 40.5 & 38.0 & 22.5 & 22.5 & 43.0 & 34.0 & 22.5 & 32.5 & 45.5 & 32.5 & 40.0 & 30.0 & 21.0 & 37.0 \\
    VideoChat \citep{videochat}        & 35.5 & 33.5 & 26.5 & 56.0 & 33.5 & 40.5 & 53.0 & 40.5 & 30.0 & 25.5 & 27.0 & 48.5 & 35.0 & 20.5 & 42.5 & 46.0 & 26.5 & 41.0 & 23.5 & 23.5 & 36.0 \\
    TimeChat \citep{Ren2023TimeChat}          & 38.5 & 40.5 & 36.0 & 61.0 & 32.5 & 53.0 & 53.5 & 41.5 & 29.0 & 19.5 & 26.5 & 66.5 & 34.0 & 20.0 & 43.5 & 42.0 & 36.5 & 36.0 & 29.0 & 35.0 & 35.0 \\
    Video-LLaVA \citep{video-llava}    & 43.0 & 46.0 & 42.5 & 56.5 & 39.0 & 53.5 & 53.0 & 48.0 & 41.0 & 29.0 & 31.5 & 82.5 & 45.0 & 26.0 & 53.0 & 41.5 & 33.5 & 41.5 & 27.5 & 38.5 & 31.5 \\
    P-LLaVA-7B \citep{pllava}          & 46.6 & 58.0 & 49.0 & 55.5 & 41.0 & 61.0 & 56.0 & 61.0 & 36.0 & 23.5 & 26.0 & 82.0 & 39.5 & 42.0 & 52.0 & 45.0 & 42.0 & \textbf{53.5} & 30.5 & 48.0 & 31.0 \\
    ShareGPT4Video \citep{sharegpt4video} & 51.2 & 49.5 & 39.5 & 79.5 & 40.0 & 54.5 & 82.5 & 54.5 & 32.5 & 50.5 & 41.5 & 84.5 & 35.5 & 62.5 & 75.0 & 51.0 & 25.5 & 46.5 & 28.5 & 39.0 & 51.5 \\
    ST-LLM \citep{st-llm}              & 54.9 & 66.0 & 53.5 & 84.0 & 44.0 & 58.5 & 80.5 & 73.5 & 38.5 & 42.5 & 31.0 & 86.5 & 36.5 & 56.5 & 78.5 & 43.0 & 44.5 & 46.5 & 34.5 & 41.5 & 58.5 \\
    VideoGPT+ \citep{videogpt+}        & 58.7 & 69.0 & 60.0 & 83.0 & 48.5 & 66.5 & 85.5 & 75.5 & 36.0 & 44.0 & 34.0 & \textbf{89.5} & 39.5 & \textbf{71.0} & \textbf{90.5} & 45.0 & 53.0 & 50.0 & 29.5 & 44.0 & 60.0 \\
    VideoChat2~\cite{mvbench} & 60.4 & 75.5 & 58.0 & 83.5 & \textbf{50.5} & 60.5 & 87.5 & 74.5 & 45.0 & 47.5 & 44.0 & 82.5 & 37.0 & 64.5 & 87.5 & 51.0 & 66.5 & 47.0 & 35.0 & 37.0 & \textbf{72.5} \\
    \midrule 
    VideoChat-TPO &\textbf{66.3} & \textbf{84.0} & \textbf{68.5} & \textbf{87.0} & 47.5 & \textbf{70.5} & \textbf{93.5} & \textbf{81.5} & \textbf{43.0} & \textbf{52.0} & \textbf{51.5} & 86.0 & \textbf{49.0} & 66.0 & 90.0 & \textbf{54.5} & \textbf{84.5} & 53.0 & \textbf{36.0} & \textbf{56.5} & 72.0 \\
    \bottomrule 
\end{tabular}
}
\label{tab:results_mvbench}
\end{table*}


==> tables/nextgqa.tex <==
\begin{table*}[ht]
% \caption{Results on NExT-GQA. Acc@IoP indicates the percentage of correct answers when the IoP $\geq$ 0.5. Acc@GQA is defined as the percentage of questions that are both correctly answered and visually grounded with IoP $\geq$ 0.5.}
  \centering
    \resizebox{0.75\linewidth}{!}{
    \begin{tabular}{l|cc|cccccc}
    \toprule
    Model &Acc@IoP &Acc@GQA &mIoP &IoP@0.3 &IoP@0.5 &mIoU &IoU@0.3 &IoU@0.5 \\
    \midrule 
    VIOLETv2 \cite{violetv2}         & 54.9 &12.8 & 23.6 & 25.1 & 23.3 & 3.1  & 4.3  & 1.3 \\  
    Temp[CLIP] NG+ \cite{nextgqa}    & 62.7 &16.0 & 25.7 & 31.4 & 25.5 & 12.1 & 17.5 & 8.9 \\  
    SeViLA \cite{sevila}             & 72.5 &16.6 & 29.5 & 34.7 & 22.9 & 21.7 & 29.2 & 13.8\\
    % VideoChat2 \citep{mvbench}     & -    & -    & -    & -    & 18.7 & 26.6 & 13.5 \\  
    LangRepo \cite{langrepo}         & 59.6 &17.1 & 31.3 & -    & 28.7 & 18.5 & -    & 12.2 \\ 
    FrozenBiLM NG+ \cite{frozenbilm} & 73.8 &17.5 & 24.2 & 28.5 & 23.7 & 9.6  & 13.5 & 6.1 \\  
    VideoStreaming \cite{streaming}  & 57.4 &17.8 & 32.2 & -    & 31.0 & 19.3 & -    & 13.3 \\  
    LLoVi  \cite{llovi}              & 65.9 &24.3 & \textbf{37.3} & -    & \textbf{36.9} & 20.0 & -  & 15.3\\  
    HawkEye \cite{hawkeye}           & -    &- & -    & -    & -    & 25.7 & 37.0 & 19.5 \\  

    % Grounded-VideoLLM~\cite{grounded-videollm}  & 77.6 &26.7 & 34.5 & 42.6 & 34.4 & 21.1 & 30.2 & 18.0 \\ 
    \midrule 
    VideoChat-TPO       & \textbf{77.7} & \textbf{25.5} & 35.6 & \textbf{47.5} & 32.8 & \textbf{27.7} & \textbf{41.2} & \textbf{23.4} \\  
    \bottomrule

\end{tabular}
}
\caption{\textbf{Performance on Grounded QA.} }%
\label{tab:results_nextgqa}
\end{table*}

==> tables/rebuttal_imagebench.tex <==
\begin{table}[ht]
  \vspace{-2mm}
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccc}
    \toprule
    Model & Seed2-I & Seed2-M & VQAv2 & MME-P & OCRBench \\ 
    \midrule
        VideoChat & 64.0 & 45.6 & 52.2 & 1201 & 76 \\ 
        % 64.0, 45.6
        VideoChat-TPO   &67.3(+3.3)& 70.0(+24.4)  & 59.6(+7.4) & 1321(+120) & 112(+36) \\
        LLaVa-OneVision  & 73.2 & 74.3 & 79.8 & 1580 & 622 \\  
        LLaVa-OneVision-TPO & \textbf{75.6}(+2.4) & \textbf{77.0}(+2.7) & \textbf{80.0}(+0.2) & \textbf{1622}(+42) & \textbf{659}(+37) \\  
    \bottomrule 
\end{tabular}
}
\vspace{-3.5mm}
\caption{\textbf{Perfermance on Image Benchmarks.}}
\label{tab:imagebench}
\end{table}

==> tables/rebuttal_visionllm.tex <==
\begin{table}[ht]
  \vspace{-2mm}
  \centering
    \resizebox{0.65\linewidth}{!}{
    % \begin{tabular}{l|ccc}
    \begin{tabular}{l|ccc}
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{3}{c}{RefCOCO+}  \\
     \cmidrule(lr){2-4}  
     & val & testA & testB \\
    \midrule
        VideoChat-TPO  & \textbf{80.2} & \textbf{85.1} & \textbf{71.7}  \\  
        VisionLLMv2  & 77.6 & 83.8 & 70.2 \\  
    \bottomrule 
\end{tabular}
}
\vspace{-3mm}
\caption{\textbf{Performance Comparison Between VideoChat-TPO and VisionLLMv2 Spatial Grounding Task}}
\label{tab:rebuttal_Refcoco+}
\end{table}

==> tables/ref_seg.tex <==
\begin{table}[ht]

    \centering
    \caption{\textbf{Zero-Shot Performance on referring segmentation.} }

    \label{tab:refvos}
    \resizebox{\linewidth}{!}{
        {
            \begin{tabular}{l | c c c | c c c}
            \toprule
            \multirow{2}*{Method} &  \multicolumn{3}{c |}{Ref-YouTube-VOS ~\cite{seo2020urvos}} & \multicolumn{3}{c}{MeViS~\cite{mevis}} \\
              & \( \mathcal{J} \)\&\( \mathcal{F} \) & \( \mathcal{J} \) & \( \mathcal{F} \)  &  \( \mathcal{J} \)\&\( \mathcal{F} \) & \( \mathcal{J} \) & \( \mathcal{F} \) \\
            \midrule
            ReferFormer~\cite{wu2022language}  & 62.9 & 61.3 & 64.6 & 31.0 & 29.8 & 32.2 \\
            OnlineRefer~\cite{wu2023onlinerefer}  &62.9& 61.0 &64.7 &- &- &-\\
            \midrule
            LISA~\cite{lai2023lisa} & 52.6 & 52.1 & 53.0 & - & - & -\\
            VideoLISA~\cite{lai2024lisa}  &63.7 & ~\textbf{61.7} &63.7 &44.4 &41.3 &47.6\\
            \midrule
            {VideoChat-TPO} & ~\textbf{63.9} &52.3 & ~\textbf{75.4} & ~\textbf{47.0} & ~\textbf{42.6} & ~\textbf{51.3} \\
            \bottomrule 
            \end{tabular}
        }
    }
    
\end{table}


==> tables/spatial_grounding.tex <==




\begin{table}[ht]
    \centering
    \caption{\textbf{Results on spatial grounding task.} The metric is \textbf{Acc@0.5}. \textcolor{gray}{$\bigstar$ refers to the specialist or fine-tuned methods.}} 
    \resizebox{0.6\linewidth}{!}{
    \begin{tabular}{l |c c c}
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{3}{c}{RefCOCO~\cite{yu2016refcoco}}  \\
     \cmidrule(lr){2-4}  
     & val & testA & testB \\
    \midrule
    % \multirow{7}{*}{non-LMM}
    \textcolor{gray}{MAttNet $\bigstar$~\citep{yu2018mattnet}} & \textcolor{gray}{76.4} & \textcolor{gray}{80.4} & \textcolor{gray}{69.3} \\
    OFA-L~\citep{wang2022ofa} & 80.0 & 83.7 & 76.4 \\
    OFASys & - & 80.1 & -   \\
    \textcolor{gray}{G-DINO-L $\bigstar$~\citep{liu2023gdino}} & \textcolor{gray}{\textbf{90.6}} & \textcolor{gray}{\textbf{93.2}} & \textcolor{gray}{\textbf{88.2}} \\
    \midrule
    VisionLLM-H~\citep{wang2023visionllm} & - & 86.7 & - \\
    Shikra-7B~\citep{chen2023shikra} & \textbf{87.0} & 90.6 & 80.2  \\
    NExT-Chat-7B~\cite{zhang2023nextchat}  & 85.5 & 90.0 & 77.9  \\
    
    \midrule
    % \midrule
     VideoChat-TPO & 85.9 & \textbf{90.8} & \textbf{81.3} \\
    \bottomrule
    \end{tabular}}
    \label{tab:rec}
\end{table}


==> tables/tracking.tex <==
\begin{table}[ht]
\centering
\large
\caption{\textbf{Performance on tracking benchmarks.}}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|ccc|ccc}
         % \setlength\tabcolsep{2pt}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{LaSOT~\cite{fan2019lasot}} & \multicolumn{3}{c}{GOT-10k~\cite{huang2019got}} \\
\cmidrule{2-4} \cmidrule{5-7}    
% \textbf{Method} 
& Success & P$_{norm}$ & P & Overlap & SR0.5 & SR0.75\\
\midrule
% \multicolumn{6}{c}{\textcolor{gray}{\emph{Single Object Tracking}}} \\
% \midrule
% \multicolumn{8}{l}{\small{\textbf{\emph{Specialist Models}}}} \\
SiamFC~\cite{siamFC}              & 33.6 & 42.0 & 33.9  & 34.8 & 35.3 & 9.8 \\
ATOM~\cite{ATOM}                 &   51.5 & -  &-  & 55.6 & 63.4 & 40.2\\
SiamRPN++~\cite{SiamRPN++}      &  49.6 & 56.9 & 49.1 & 51.8 & 61.8 & 32.5\\
SiamFC++~\cite{SiamFC++}          &  54.4 & 62.3 & 54.7 & 59.5 & 69.5 & 47.9\\
\midrule    
% \multicolumn{8}{l}{\small{\textbf{\emph{Generalist Models}}}} \\
LLaVA-1.5~\cite{llava}  & 19.4 & 16.5 & 12.8 & 23.5 & 20.2 & 9.7 \\
Merlin~\cite{yuen2023merlin}  & 39.8   & 40.2  & 38.1 & 51.4 & 55.9 & 42.8\\
\midrule
VideoChat-TPO  & \textbf{69.4}  & \textbf{80.1}  & \textbf{76.9} & \textbf{70.6} & \textbf{79.8} & \textbf{66.0}\\
\bottomrule
\end{tabular}
}
% \setlength{\abovecaptionskip}{0.15cm}
\label{tab:track}
% \vspace{-3mm}
\end{table}


==> tables/videomme.tex <==
\begin{table}[ht]
\caption{Performance comparison of MLLMs on Video-MME. w/o s. means without subtitle and w s. means with subtitle. F indicates the number of frames.}
  \centering
  \resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|cc|cc|cc|cc}
    \toprule
    
    \multirow{2}{*}{Model} &  \multirow{2}{*}{F} & \multicolumn{2}{c}{Overall}
    & \multicolumn{2}{c}{Short } & \multicolumn{2}{c}{Medium } & \multicolumn{2}{c}{Long }\\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6}  \cmidrule(lr){7-8} \cmidrule(lr){9-10} 
    &  & w/o s.  & w s. & w/o s.  & w s. & w/o s.  & w s. & w/o s.  & w s. \\  
    \midrule 
    VideoChat2~\cite{mvbench}  & 16  & 39.5 & 43.8 & 48.3 & 52.8 & 37.0 &39.4 &33.2 &39.2\\ 
    Video-LLaVA~\cite{video-llava} & 8 & 39.9 & 41.6 &45.3&46.1& 38.0& 40.7 & 36.2 & 38.1\\  
    ST-LLM~\cite{st-llm}   & 64   & 39.9 & 43.6  & 45.7 & 48.7 & 36.8 & 41.4 & 31.3 & 36.9\\ 
    Chat-UniVi~\cite{jin2023chatunivi} & 64 & 40.6&	45.9  & 45.7 & 51.2 & 40.3 & 44.6 & 35.8 & 41.8\\
    ShareGemini~\cite{ShareGemini} &64 & 43.2 &47.9 & 49.1 & 52.8 & 41.3 & 47.3 & \textbf{39.1} & 43.4\\
    \midrule 
    VideoChat-TPO & 16  &\textbf{46.2} & \textbf{51.5}  & \textbf{54.9} & \textbf{60.8} & \textbf{42.6} & \textbf{48.0} & \textbf{41.1} & \textbf{45.8}\\ 
    \bottomrule
    \end{tabular}
}
\label{tab:videomme}
\end{table}

